Deep Watershed Transform for Instance Segmentation

Most contemporary approaches to instance segmentation use complex pipelines involving conditional random fields, recurrent neural networks, object proposals, or template matching schemes. In our paper, we present a simple yet powerful end-to-end convolutional neural network to tackle this task. Our approach combines intuitions from the classical watershed transform and modern deep learning to produce an energy map of the image where object instances are unambiguously represented as basins in the energy map. We then perform a cut at a single energy level to directly yield connected components corresponding to object instances. Our model more than doubles the performance of the state-of-the-art on the challenging Cityscapes Instance Level Segmentation task.

==> dist.tex <==
%!TEX root = top.tex

\section{Distance Transform}

Choosing the proper training target and loss function is critical to the performance of a convolutional neural network model whose parameters are determined by gradient descent optimization methods. Ideally, the derivative of a defined loss with respect to each weight should be a robust signal over a wide range of inputs and weight initializations without diminishing or saturating. Moreover, it is important that the phrasing of the training target is such that the network's overall objective is encoded as clearly as possible. This section presents the intuition behind and development of our architecture and training procedure, following the above principles. 

The instance-aware distance transform of a scene is a scalar field where the value at each pixel is the euclidean distance to the nearest pixel outside of the instance containing said pixel. Thus the distance transform $D(p)$ for points $p$ in object $o$ covering pixels $\{p_o\}$ can be expressed by equation \ref{eq:dist_transform}. 

\begin{equation} \label{eq:dist_transform}
\text{D}(p) = \min_{p' \not\in \{p_o\}} \|p-p'\|^2
\end{equation}

Moreover, we can find the unit vector of the gradient of the distance transform $D'(p)$ as in equation \ref{eq:unit_vec}

\begin{equation} \label{eq:unit_vec}
\vec{u}_p =  \frac{[ \frac{D_x(p)}{dx}, \frac{D_y(p)}{dy}]}{\| [\frac{D_x(p)}{dx}, \frac{D_y(p)}{dy}]\|^2}
\end{equation}

The angle represented by $\vec{u}_p$ can be easily found. Figure \ref{fig:dist_intro} illustrates these transformations. 

The original instance labelling gives homogeneous labels to pixels within each object, and is not directly useful for training a network. On the other hand, the distance transform provides a different value for each pixel. The connected components in the thresholded output immediately yields all object instances. This indirectly encodes the presence of object boundaries. However, the network must simultaneously learn to recognize boundaries and discover the distance transform function. 

The angular image encodes the most direct signal regarding boundaries and presents a simpler task. For each pixel, it is only necessary to predict a direction away from the nearest region not belonging to the containing object. Moreover, for a pair of pixels straddling an object boundary, the difference between their corresponding angles is at the maximum possible value of 180$^{\circ}$. This presents the greatest level of cost possible for associating a pixel near an instance boundary with the wrong object instance. 

\begin{figure*}[t]
\begin{center}

\begin{subfigure}[b]{0.250\textwidth} \centering \includegraphics[width=\textwidth]{figures/dist/inst.png} \end{subfigure}
\begin{subfigure}[b]{0.250\textwidth} \centering \includegraphics[width=\textwidth]{figures/dist/dist.png} \end{subfigure}
\begin{subfigure}[b]{0.250\textwidth} \centering \includegraphics[width=\textwidth]{figures/dist/dir.png} \end{subfigure}

\caption{From left to right: a) instance level segmentation, b) distance transform $D(p)$, c) angle of $\vec{u}_p$}\label{fig:dist_intro}
\end{center}
\end{figure*}
